Distributed Methods for High-dimensional and Large-scale Tensor Factorization

Given a high-dimensional large-scale tensor, how can we decompose it into latent factors? Can we process it on commodity computers with limited memory? These questions are closely related to recommender systems, which have modeled rating data not as a matrix but as a tensor to utilize contextual information such as time and location. This increase in the dimension requires tensor factorization methods scalable with both the dimension and size of a tensor. In this paper, we propose two distributed tensor factorization methods, SALS and CDTF. Both methods are scalable with all aspects of data, and they show an interesting trade-off between convergence speed and memory requirements. SALS updates a subset of the columns of a factor matrix at a time, and CDTF, a special case of SALS, updates one column at a time. In our experiments, only our methods factorize a 5-dimensional tensor with 1 billion observable entries, 10M mode length, and 1K rank, while all other state-of-the-art methods fail. Moreover, our methods require several orders of magnitude less memory than our competitors. We implement our methods on MapReduce with two widely-applicable optimization techniques: local disk caching and greedy row assignment. They speed up our methods up to 98.2X and also the competitors up to 5.9X.

==> 070related.tex <==
\textbf{Coordinate Descent.}
Coordinate descent is a classic optimization method which updates one parameter at a time while keeping others fixed.
It has been applied to diverse data mining algorithms including nonnegative matrix factorization \cite{cichocki2009fast, hsieh2011fast}, matrix factorization for recommendation \cite{yu2013parallel, DBLP:conf/icdm/YuHSD12}, and linear SVMs \cite{hsieh2008dual}.
It also has been applied to nonnegative tensor factorization \cite{cichocki2009fast, liu2012sparse}, but existing methods cannot be used for recommendation and have limited scalability because they assume that all the entries of a tensor are observable.

\textbf{Matrix Factorization.}
Matrix factorization (MF) has been successfully used in many recommender systems \cite{chen2011linear, koren2009matrix, zhou2008large}.
The underlying intuition of MF for recommendation can be found in \cite{koren2009matrix}.
Two representative approaches for large-scale MF are alternating least squares (ALS) and stochastic gradient descent (SGD).
ALS is inherently parallelizable \cite{zhou2008large} but has high memory requirements and computational cost \cite{DBLP:conf/icdm/YuHSD12}.
Efforts have been made to parallelize SGD \cite{gemulla2011large, mcdonald2010distributed, zinkevich2010parallelized}, and distributed stochastic gradient descent (DSGD) \cite{gemulla2011large} divides a matrix into disjoint blocks and processes them simultaneously. %, is most successful.
Recently, coordinate descent also has been applied to large-scale MF \cite{yu2013parallel, DBLP:conf/icdm/YuHSD12}.

\textbf{Tensor Factorization.}
A comprehensive survey on tensor factorization can be found in \cite{kolda2009tensor}.
The factorization of partially observable tensors has been used in various fields including computer vision \cite{liu2013tensor}, chemometrics \cite{tomasi2005parafac}, social network analysis \cite{dunlavy2011temporal}, and Web search \cite{sun2005cubesvd}.
Recently, it also has been used for recommendation \cite{Karatzoglou:2010, nanopoulos2010musicbox, zheng2010collaborative} as additional information such as time and location has become available.
For efficient PARAFAC decomposition, distributed algorithms \cite{beutel2014flexifact} as well as serial algorithms \cite{acar2011scalable, tomasi2005parafac} have been proposed.

\textbf{\MR and Hadoop.}
\MR \cite{dean2008mapreduce} is a distributed computing framework for processing Web-scale data.
A variety of data mining algorithms, including matrix factorization \cite{gemulla2011large} and tensor factorization \cite{beutel2014flexifact}, have been implemented on \MR.
Nevertheless, its limited computational model and inefficiency because of the repeated distribution of data have been pointed out as problems \cite{teflioudi2012distributed, DBLP:conf/icdm/YuHSD12}, which are partially resolved in this paper by direct communication and local disk caching, respectively.
Hadoop \cite{Hadoop} is an open-source implementation of \MR and is widely used in both academia and industry owing to its scalability and utility. 

==> ACK-cta.tex <==

\thanks{
This material is based upon work
   supported by the National Science Foundation
   under Grants No.
%   DBI-0640543 % with Eric - for Lei and Fan - fly embryos
   IIS-0705359 and % tensors, - for Babis and U Kang - with Vasilis
%   CNS-0721736 % bgp with Michalis - for Aditya and Polo
   IIS0808661, % nematodes with UCR - for Mary, Leman and U Kang
%   IIS1017415 % virus prop., with Hanghang and Aditya
%   IIS0970179. % EAGER grant, with Humanities colleagues from UCLA and UCB
%   Also
%   iCAST % with Taiwan - for Leman, Lei, Babis, Aditya
   %% and under the auspices of the U.S. Department of Energy
   %% by University of California Lawrence Livermore National Laboratory
   %% % for 2008 or earlier
   %% % under contract No.W-7405-ENG-48.
   %% % under contract DE-AC52-07NA27344 (LLNL-CONF-404625),
   %% % subcontracts B579447, B580840.
   %% %
   %% % for 2009-2010
   %% under contract DE-AC52-07NA27344
   % This work was performed
   % for 2010, for Hanghang, Lei, Leman
%   and under the auspices of the U.S. Department of Energy by Lawrence
%   Livermore National Laboratory under contract
%   # No. DE-AC52-07NA27344.
%   B594252 # for 2011 - this is for Lei
%
   % DTRA grant with Abdelzaher, Eliassi-Rad, Han - for U Kang,
%   Research was sponsored
%
   by the Defense Threat Reduction Agency
   under contract No. HDTRA1-10-1-0120,
%
   % for work on the ARL CTA grant with UIUC - Aditya, Leman, U
%   Research was sponsored
%
   %,
   and by the Army Research Laboratory
   and was accomplished under Cooperative Agreement Number W911NF-09-2-0053.
   This work is also partially supported by
   an IBM Faculty Award, and the Gordon and Betty Moore Foundation, in the eScience project.
   The views and conclusions contained in this document are those
   of the authors and should not be interpreted as representing
   the official policies, either expressed or implied,
   of the Army Research Laboratory, the U.S. Government, or the National Science Foundation.
   The U.S. Government is authorized to reproduce and
   distribute reprints for Government purposes notwithstanding
   any copyright notation here on.


   % a Google Focused Research Award,
   % a Yahoo Research Alliance Gift,
   % a SPRINT gift,
   % with additional funding from Intel, NTT and Hewlett-Packard.
%   Any opinions, findings, and conclusions or recommendations expressed in this
%   material are those of the author(s) and do not necessarily reflect the views
%   of the National Science Foundation, or other funding parties.
}


